From Who You Know to What You Read: Augmenting Scientific Recommendations with Implicit Social Networks

The ever-increasing pace of scientific publication necessitates methods for quickly identifying relevant papers. While neural recommenders trained on user interests can help, they still result in long, monotonous lists of suggested papers. To improve the discovery experience we introduce multiple new methods for \em augmenting recommendations with textual relevance messages that highlight knowledge-graph connections between recommended papers and a user's publication and interaction history. We explore associations mediated by author entities and those using citations alone. In a large-scale, real-world study, we show how our approach significantly increases engagement -- and future engagement when mediated by authors -- without introducing bias towards highly-cited authors. To expand message coverage for users with less publication or interaction history, we develop a novel method that highlights connections with proxy authors of interest to users and evaluate it in a controlled lab study. Finally, we synthesize design implications for future graph-based messages.

==> src1_intro_alt1.tex <==
% Highlight the difference 


% \hyeonsu{Describe why we care about the scientific recommendations in a paragraph, and get to the interesting findings from our studies}
Research in explainable recommendations (see~\cite{zhang2018explainable} for an extended review) and theories of social influence and social proof~\cite{cialdini2009influence} suggest that our preferences can be altered by information about the recommended items and the actions of those around us. As a result, approaches that use relevance information to augment and explain recommendations are pervasive in recommender systems in the domains of e-commerce~\cite{he2015trirank,wang2018explainable}, music~\cite{sharma2013social,zhao2019personalized}, blogs~\cite{zhao2014we}, social networks (e.g., Facebook and Twitter), movies~\cite{herlocker2000explaining,tintarev2008effectiveness}, videos~\cite{toderici2010finding}, and books~\cite{wang2018ripplenet} and so on~\cite{tintarev2007survey,andersen1989hugin,bilgic2005explaining,buchanan1984rule}. Missing the domain of scientific recommendations in the literature, a natural follow-up question is whether similar approaches for producing explainable recommendations can be applied to this new domain, and how they might change or not change user preferences and information behavior.\jb{I don't find the domain difference compelling on its own - better to highlight new findings from our study, method for scaling author-mediated connections, etc}

Scientific recommendations is a particularly interesting domain for three main reasons. The first reason is existing user needs \jb{Don't other domains have existing user needs too?} from researchers who face the problem of information overload~\cite{case2016looking,miller1960information} due to the immense scale and dynamic changes of human knowledge in the archival literature~\cite{jinha2010article,bornmann2015growth,noorden_doubling_output,tenopir2009electronic,rowland2002overcoming}. In order to exploit the wealth of knowledge without getting overwhelmed, researchers have developed tailored strategies such as skimming, power browsing, and squirrelling~\cite{rowlands2008google,nicholas2010researchers,vilar2015information}. They also frequently turn to social networks (e.g., Twitter and Academia.edu), and adopt RSS feeds or email alerts to receive personalized recommendations~\cite{van2014online,watkinson2016changes,tenopir2019changes}. Nonetheless, these solutions are still piecemeal and tedious, and relied upon chance discovery~\cite{breitinger2019too}. 

Another reason arises from a unique epistemic state of being that is different from other application domains of explainable recommendations. In our hyper connected world with no single mind that contains the entirety of archival knowledge, researchers must depend on others~\cite{bromme2010knows} to make judgement on scientific recommendations. Unlike previous application domains of explainable recommendations where users could easily interact with the recommended items to make their own judgment, the division of cognitive labor characteristic to scientific recommendations may reduce users' ability of making effective or equally confident judgment, and raises a question of feasibility for existing approaches, whether their effectiveness may similarly transfer to effect changes on epistemic preferences. The domain of scientific recommendations is further differentiated by other factors such as the lack of researchers' knowledge~\cite{bromme2014public,zimmermann2018experts}, conflicting claims in the literature~\cite{stadtler2014content}, and the interrelated processes of trust, intent, and knowledge in learning and scientific reasoning~\cite{landrum2015learning}. Recently, there has been a line of research on designing new incentive mechanisms for open science initiatives such as visual badges awarded for research articles that share data or code publicly for reproducibility to encourage researchers' behavior changes~\cite{rowhani2020did,schweitzer2018open}. Our work is similar to this line of research in terms of the domain and the empirical approach taken (i.e. randomized online study involving researchers), but also differs in terms of the goal which is increasing researchers' preference and engagement with research article recommendations, rather than incentivizing long term behavior changes.

Lastly, there are unique features of scientific recommendations that provide us an opportunity to design novel relevance messages. One such feature is the citation graph that makes visible how new research articles build on the existing literature. Using references of new incoming paper recommendations for example we can surface connections to existing papers that the user authored or liked before, and leverage them as to indicate relevance. Alternatively, because the authors of paper recommendations are also similarly connected and mediated by the citation graph, we can surface salient and relevant author-focused connections to indicate relevance. Such mechanisms may also generalize to other domains with similar properties, such as patents or legal cases.

Given these distinctions, we are motivated by the question: \textit{Can at-a-glance relevance information augmenting personalized paper recommendations enhance researcher engagement and sensemaking?} This work takes a series of steps to uncover generalizable design implications for different types of at-a-glance relevance information, by focusing on the specific use context of paper recommendations received in user-subscribed email alerts. At a high level, there are contrasting notions of relevance in the literature on information need and perceived value of scholarly articles~\cite{case2016looking,belkin1985interaction} which we distinguish first. The logical notion of relevance, construed as aboutness or topicality (i.e. is the article on an appropriate topic as evidenced by containing specific terms?) differs from the user's situational relevance which often emphasizes the notion of personalized usefulness. While the former focuses on content relatedness, the latter centers around users' subjective usefulness and broader information needs, which extend beyond the need for maximal content relatedness. For example, a researcher might find paper recommendations \textit{relevant} not because their content is directly related to a predefined research topic but because they are building off of the researcher's prior work, which she finds useful for understanding her work's impact in the field and ideating future research directions. Alternatively, she might find paper recommendations \textit{relevant} because of her social connection with one of the authors, as she is curious about what current and former colleagues are working on, and having a high-level understanding of their research trajectories gives her ideas for discussion, even if they are topically divergent. In yet another example, she might find paper recommendations useful because of the new authors she discovered from them, who she otherwise would not have encountered or paid enough attention to notice. As will be shown later, all of these examples involve usefulness outside the first notion of direct content relevance. In order to support such types of information needs, this work takes the broader, second perspective of relevance.

In this paper, we introduce three kinds of graph-based relevance explanations. The first kind (Citation-based relevance) was motivated by how researchers use bibliographic connections to search through the `back chains' of relevant prior work~\cite{barrett2005information,covi1999material,vakkari2006searching,westbrook2003information,bates2002speculations} and computes relevance via citation graphs of papers (e.g., ``This paper also cites 3 of your papers.''). The nodes of the graph are papers, either the user authored or previously expressed interest for, for example by saving them in the personal library or clicking the `thumbs up' buttons. The links in the graph are mapped from pairwise incoming (citations) and outgoing (references) connections between papers. Unlike older articles, the newly published paper recommendations are often one-sided in their connections to other papers in the graph, with few incoming citations but potentially a number of references included in them; therefore, we use reference links to model relevance.

The second kind (Direct author-based relevance) presents relevance via author graphs (e.g., ``You cited this author 4 times.''), constructed by replacing each paper node in the citation graph with a set of author nodes and linking them by mirrored paper connections from the citation graph. This kind was motivated by how researchers currently follow work from a set of researchers known to them, for example on social media platforms such as Twitter or Academia.edu. The author-based relevance is similar to prior work in social explanations for other domains~\cite{sharma2013social,wang2014also} which uses friendship relationship among the users and their preferences on recommended items to generate relevance messages. However, our author graph differs in terms of the relational semantics (i.e. cited authors vs. friendship) and implications on data privacy. Unlike publicly available citation information, a user's friends' preferences remain as private information even for the user herself. 

This paper begins with an iterative design process that involved several rounds of prototyping and informal evaluation with internal users and several relevant stakeholders. In total the process involved 7 users, a designer, a marketing person, and 3 researchers in the fields of Artificial Intelligence and Human-Computer Interaction. This iterative process resulted in the final message template designs for the first two types of relevance (citation- and direct author-based, Section~\ref{xx}). The message templates were filled in with personalized data and used to augment paper recommendations in new paper email alerts sent to users who subscribed to them. Given its use context, our message design's goals included brevity, visibility, and understandability. The final design (fig.~\ref{fig:xx}) adopted distinctive visual elements and colors, and was placed under each paper recommendation for easy access and low overhead for skimming.

We then describe the procedure of a randomized online study which sought evidence for the feasibility of citation- and direct author-based relevance messages. While conducting design iterations and informal interviews provided initial qualitative insights into how relevance messages might support user engagement with new research article recommendations, without a large scale randomized experiment we were not able to quantify exactly how effective such methods might be. In order to examine this, we ran a randomized online experiment with more than seven thousand users on a popular scholarly search engine over a two-month-long period, by deploying personalized paper recommendations and relevance messages to alert email subscribers who were randomly assigned to each of the three conditions (Control vs. Citation-based vs. Direct author-based). Our result showed that both types of relevance messages significantly increased user engagement over Control, and that author-based relevance messages were more effective than citation-based relevance message: 268\% (author-based) and 159\% (citation-based) increase on the fraction of clicked emails that featured at least one relevance message of each type. Moreover, author-based relevance messages also resulted in a higher email open rate (13\% increase over Control), but not citation-based messages.

%24\% and 29\% increase over Control on the binary email click rates -- i.e. at least one click in the email -- using citation- and direct author-based messages, respectively. 

However, the effectiveness of relevance messages was hindered by their low frequency, and author-based messages were scarcer despite its effectiveness, with only less than 4\% of paper recommendations in alert emails featuring relevance messages (in comparison, citation-based messages were significantly more common at around 9\%). In follow-up analyses using logistic regression, we show that this scarcity of relevance messages indeed seemed to prevent broader engagement from users. To scale the effective author-based relevance messages, we designed and implemented a new kind of relevance messages (Indirect author-based relevance) that presents relevance via [author]-[trusted author]-[user] triplet relations on author graphs (e.g., ``This author is often cited by an author you give credit to.''). In other words, the indirect author-based relevance incorporated `endorsement' from a known intermediate author who the user may trust and would appreciate paper recommendations from. To enable this relevance, we expanded exploration on the author graph to second-degree relations, while separately inferring a list of intermediate, trusted authors from users. The choice of intermediate authors included: authors whose publications are highly relevant to those of the user; authors who frequently co-authored with or were cited by the user; and authors of papers the user frequently liked or saved in the personal library. %The presentation of this message included both a description of the connection between the user and the intermediate author as well as a description of the connection between the intermediate author and the author of the recommended paper.

Then, we compared all three kinds of relevance messages and Control in a controlled user study with fourteen researchers (Section~\ref{xx}). Researchers were observed as they reviewed paper recommendations augmented with relevance messages. Using open coding of the interviews, we found qualitative insights into different types of usefulness that our relevance messages provided, which complemented the quantitative results from Study One. Some of the types of usefulness included: discovering new information about self and other authors to learn more; vetting potential usefulness of paper recommendations; mobilizing mental models of prior work and author expertise to better understand the recommendations; and as a general aid that increases user attention to others' work which was perceived useful for users' broader social context. We also uncover several design implications for future approaches using similar graph-based relevance messages for scientific recommendations including: the tension between increased context and efficiency of skimming; adapting to users' evolving identities as researchers; and the challenges related to diffusion of relevance.

In summary, this work makes five contributions. First, we designed and implemented two types of relevance messages augmenting personalized paper recommendations, grounded in an iterative design process and informal interviews with multiple stakeholders. Second, we present evidence from a large scale online deployment study that our augmentation approach indeed increases user engagement in the domain of scientific recommendations, and that author-based relevance messages perform better, although its full potential is not likely reached due to the low frequency. Third, we design and implement an additional kind of relevance messages that models endorsement from intermediate authors that users likely know and give credit to, in order to offset the limitation from the scarcity of messages. Fourth, we provide qualitative insights into how different types of relevance messages benefit users from a controlled lab study with fourteen researchers. Finally, we uncover design implications for future augmentation approaches that aim to incorporate relevance information.

\jb{Would be nice if we could explain how people who don't care about scholarly literature discovery can use our findings}

==> src1_intro_alt2.tex <==
% Highlight the difference 

Explaining how recommendations are relevant to users is critical for engagement and has been widely studied in many domains~\cite{he2015trirank,wang2018explainable,sharma2013social,zhao2019personalized,zhao2014we,herlocker2000explaining,tintarev2008effectiveness,toderici2010finding,wang2018ripplenet,tintarev2007survey,andersen1989hugin,bilgic2005explaining,buchanan1984rule,zhang2018explainable}. Scientific recommendation is a particularly interesting domain for relevance explanations given the significant influence it has on scientists' decision-making around what they should read next and which authors they should pay attention to. More and more researchers also increasingly subscribe to recommendation services like RSS feeds or curated email alerts to receive personalized recommendations~\cite{watkinson2016changes,tenopir2019changes}, hoping that such services would greatly reduce their fear of missing out on important new advances in the field and the anxiety from being overwhelmed by the torrent of information~\cite{woolston2019phds,williams2019postgraduate,hemp2009death}. Ironically, these services fall short of the vision due to impoverished information of relevance which leaves the researchers wondering to what they should pay their limited attention and why. Yet, it is unclear what kinds of information researchers might find useful to see featured in relevance explanations, how that information might be effectively communicated, and what might be the broader challenges and design implications for relevance explanation in the domain of scientific recommendations.

We are motivated by the question: \textit{Can at-a-glance relevance information augmenting personalized paper recommendations enhance researcher engagement and sensemaking?} This work takes a series of steps to uncover the benefits and challenges related to the class of approaches for explaining scientific recommendations in a model-agnostic, post-hoc manner~\cite{zhang2018explainable}, in an email alert setting where users curate interesting research articles and opt-in to receive emails that contain new research articles related to their interest on a regular basis. This task context is realistic given related studies on scholarly information behaviors and researchers' current needs~\cite{van2014online,watkinson2016changes,tenopir2019changes,breitinger2019too} and has far-reaching practical implications given the popularity of scholarly recommender systems. The task scenario also brings a set of characteristics specific to its context, for example the challenge of information overload in the face of an immense scale and dynamic changes in archival literature~\cite{case2016looking,miller1960information,jinha2010article,bornmann2015growth,noorden_doubling_output,tenopir2009electronic,rowland2002overcoming}, the prevalence of tailored strategies that users adopt to cope with this challenge such as skimming, power browsing, and squirrelling~\cite{rowlands2008google,nicholas2010researchers,vilar2015information}, and the complex network of relations existing between researchers and papers. These characteristics inform us of the unique constraints and resources that we can leverage to address the question.

In addition, what researchers may consider as relevant depends on their information need and perceived value of research papers~\cite{case2016looking,belkin1985interaction}. The {\em logical} notion of relevance, construed as aboutness or topicality (i.e. is the article on an appropriate topic as evidenced by containing specific terms?) differs from the user's {\em situational} relevance which often emphasizes the notion of personalized usefulness. While the former focuses on content relatedness, the latter centers around users' subjective usefulness and broader information needs, which extend beyond the need for maximal content relatedness. For example, a researcher might find paper recommendations \textit{relevant} not because their content is directly related to a predefined research topic but because they are building off of the recommended researcher's prior work, which she finds useful for understanding her work's impact in the field and ideating future research directions. Alternatively, she might find paper recommendations \textit{relevant} because of her social connection with one of the authors, as she is curious about what current and former colleagues are working on, and having a high-level understanding of their research trajectories gives her ideas for discussion, even if they are topically divergent. In yet another example, she might find paper recommendations useful because of the new authors she discovered from them, who she otherwise would not have encountered or paid enough attention to notice. As will be shown later, all of these examples involve usefulness outside the first notion of direct content relevance. 

This work aims at supporting the situational relevance and the associated information needs for researchers through graph-based relevance explanations. Unlike logical relevance, this type of relevance may not be directly accessible from the content and metadata of papers alone, and especially scarce for new paper publications common in our task setting which lack incoming citations and metadata. To overcome these limitations, we propose two kinds of graph-based relevance messages based on citation-graphs and the inferred social networks of authors. A core distinction between our approaches and prior work in recommender systems and literature search tools that proposed graph-based algorithms~\cite{catherine2016personalized,chaudhari2017entity,ostuni2013top,bethard2010should,chen2010short} is that we use graphs strictly to generate useful relevance messages that support information needs in the situational sense, independent of the underlying recommender systems used to generate the recommendations. Furthermore, we use a novel approach of inferring social networks of authors implicit in citation-graphs to generate author-based relevance messages. The most conceptually similar prior work to our second, author-based relevance messages is Sharma and Cosley~\cite{sharma2013social} which studied the effectiveness of social explanations in music recommendations. However, an open question remains as to whether and how prior work that relied on existing social networks to surface socially grounded connections could be adapted to scientific recommendations where no explicit social networks exist, and connections through citation networks might not be grounded in the social world.

%% Hyeonsu actively working on this 
% In order to support such types of information needs, this work takes the broader, second perspective of relevance.\jb{What does it mean to take the situational relevance perspective - does this exclude ``logical''}

% \jb{Relatedly, Why do we focus on graph-based relevance messages - because this information is not visible, whereas logical relevance can be determined from reading paper metadata? Also relevant - these are the two types of citation relations that apply to new papers (which don't typically have incoming citations and for which we typically don't have venue info)}

% This work introduces two kinds of graph-based relevance messages based on citation-graph and the implicit social network\jb{Connect social networks better with prior paragraph - in title; important framing} of authors connected through the citation graph. Previously graph-based algorithms have been proposed in recommender systems to improve recommendations~\cite{catherine2016personalized,chaudhari2017entity,ostuni2013top}, or to jointly produce more interpretable explanations of how the recommendations were generated. Citation-graphs have also been used to improve literature search~\cite{bethard2010should}. Our approach of relevance messages differs from prior work on recommendation explanations in its construction phase (messages are generated post-hoc and independent of how recommendations were generated), motivation (searching through the `back chains' of relevant prior work is a manual process for many researchers~\cite{barrett2005information,covi1999material,vakkari2006searching,westbrook2003information,bates2002speculations}), and the goal (support the broader notion of relevance for sensemaking and discovery). The most conceptually similar prior work to our second, author-based relevance messages is Sharma and Cosley~\cite{sharma2013social} which augmented randomly selected musicians with different kinds of social explanations. Our work differs from this work in that instead of leveraging the existing social network of friendship relations, we infer a network of author relations from the citation-graph. 
%\jb{This paragraph reads like a related work paragraph. We don't need to describe all the work that uses KGs to improve explanations. Did Sharma and Cosley solve our problem - what are the open questions?}

%%%% hyeonsu actively working on this

Through an iterative design process involving several stakeholders, we developed robust message designs for use in a randomized online experiment with over \fnum{7000} users on a popular scholarly search engine, conducted over a two-month-long period. Participants who opted in for the experiment received either regular new paper recommendation emails without relevance messages (Control), emails with citation-based relevance messages (Citation-based), or emails with author-based relevance messages (Direct author-based). The result showed a significant increase in user engagement with emails augmented with graph-based relevance messages, and specifically author-based messages showed the highest increase on the fraction of clicked emails over Control (268\% increase). Author-based relevance messages also seemed to result in a higher level of future engagement, with 13\% increase over Control in the email open rates. Furthermore, through an analysis of the distribution of clicked paper recommendations, we found that user engagement did not shift to papers written by authors with higher academic status in the author-based relevance message condition compared to Control, suggesting that the messages were unlikely to exacerbate the \textit{rich-get-richer} phenomenon~\cite{merton1968matthew}. 

However, the effectiveness of author-based relevance messages was limited by their scarcity; they increased engagement beyond citation-based relevance messages despite occurring much less frequently. Less than 4\% of paper recommendations in alert emails featured author-based relevance messages. In comparison, citation-based messages were significantly more common at around 9\%. In follow-up analyses using generalized linear mixed models, we show that increasing the fraction of paper recommendations featured with author-based relevance messages is likely effective for further engaging the users. To achieve this, we designed and implemented a novel indirect author-based relevance messages, which expand the scope of author graphs by incorporating trusted and familiar middle authors in [author]-[trusted author]-[user] triplet relations (e.g., ``This author is often cited by an author you give credit to.''\jb{Can we use an example that is in our actual class of messages}).  In other words, the indirect author-based relevance incorporated `endorsement' from a known intermediate author who the user may trust and would appreciate paper recommendations from.

From a controlled lab study with fourteen researchers, we show the feasibility of indirect author-based messages for increasing the coverage and featuring familiar indirect authors in the message that users can recognize to make sense of the relevance conveyed in the message. In addition, we gained qualitative insights into different types of benefits and challenges involved with relevance messages. At a high-level, the benefits can be classified into two categories. The first category is benefits directly \textit{on} recommendations, such as mobilizing their mental models of authors to gain a deeper understanding of recommended papers, or judging the potential usefulness of them. The second category of benefits was rather \textit{around} the recommendations, such as keeping tabs on researchers they care about, understanding connections within academic communities, and understanding one's impact in the academic community. These findings confirm results from prior studies that cast recommendation as a socially embedded process that depends on both trust and the relationship of individuals~\cite{lueg1997social,perugini2004recommender}, but also surface new factors and design implications specific to scientific recommendations situated in a broader intellectual community. 

%confirm our hypothesis about how the notion of relevance may be construed broadly in scientific recommendations, and 


In summary, this work makes five contributions. First, we designed and implemented two types of graph-based relevance messages augmenting personalized paper recommendations, grounded in an iterative design process and informal interviews with multiple stakeholders. Second, we present evidence from a large-scale online deployment study that our messaging approach indeed increased user engagement, and that author-based relevance messages performed better, although its full potential was likely not reached due to low coverage. Third, we designed and implemented an additional, indirect author-based message that models endorsement from known intermediate authors that users likely give credit to, in order to mitigate the scarcity issue of author-based relevance messages. Fourth, from a controlled lab study with fourteen researchers, we showed the feasibility of indirect author-based relevance messages and presented qualitative insights into how different types of relevance messages benefited users. Finally, we uncovered design implications for future augmentation approaches that aim to incorporate graph-based relevance information.



==> src1_intro_old.tex <==
% Explanation of how a research article relates to a scholar's own work helps align the incentive of search\jb{Tangent? we don't study search} (e.g., ``how can \textit{I} build off of this result?''\jb{Poor example - we don't support this Q}) and provides benefits to scholarly sensemaking and discovery. Yet the information of relevance\jb{unclear definition} is not always recognizable from the article itself, is cumbersome to acquire, and as a result, reduces the researcher's engagement. In order to enrich relevance among the articles they encounter, researchers rely more than ever on tools such as RSS feeds, social media, and email alerts to curate relevant papers and receive recommendations~\cite{van2014online,watkinson2016changes,tenopir2019changes}\jb{Unclear how these help enrich relevance - aren't these just different paper rec channels?}. In turn, such tools are generally perceived by researchers as great channels for receiving up-to-date information on advances in related fields~\cite{van2014online}. 


% However, the increasing scale and complexity of the scientific literature (e.g., one estimated more than 50 million articles to have been published by 2009, and the number continues to grow at an exceedingly fast rate~\cite{jinha2010article})~\cite{bornmann2015growth,noorden_doubling_output,tenopir2009electronic} poses a threat of information overload~\cite{case2016looking,miller1960information} to researchers who wish to leverage such tools to stay on top of the related literature. Though existing tools dramatically increased the coverage of potentially relevant prior research, the availability of relevance information has mostly remained constant, creating a bottleneck. Researchers find the process of maintaining trusted sources of scholars often tedious, scattered, and relies on serendipitous discovery~\cite{breitinger2019too}. In addition, the popularity of tailored strategies in response to the immense scale of the literature such as skimming, power browsing, and squirrelling~\cite{rowlands2008google,nicholas2010researchers,vilar2015information} suggests that the challenge of information overload is made even more difficult now due to the limited time and attention given to processing each article.\jb{This paragraph doesn't tell me how existing tools fall short (of solving what problem? still unclear) - mostly it is more motivation about the scope/importance of the general challenge of keeping up to date, which is background that might best go at beginning of 1st para}


%%% Hyeonsu trying an alternative framing
% \hyeonsu{trying an alternative framing}
% * Main difference from other works in social explanations (e.g., Sharma and Cosley) is that the nodes in the graph are `prosumers' in nature, as opposed to being content consumers only. Examples of such networks abound:  including academic networks, where scholars both receive and author papers; sharing economy (AirBnB, where users may be interested in receiving recommendations of accommodation options as well as advertising their own; open software?; DIY community? Recommendation explanations 


%%%



The immense scale and dynamic changes of human knowledge in the archival literature~\cite{jinha2010article,bornmann2015growth,noorden_doubling_output,tenopir2009electronic} has an interesting duality: as a source for infinite possibilities of innovations and as a fire hose of information that overloads researchers who wish to stay on top of the relevant literature. In order to exploit the wealth of knowledge while mitigating the challenge of information overload~\cite{case2016looking,miller1960information}, researchers have developed tailored strategies such as skimming, power browsing, and squirrelling~\cite{rowlands2008google,nicholas2010researchers,vilar2015information}. At the core, these strategies implement a similar mechanism: reducing the amount of time and attention given to each article in order to increase the researcher's bandwidth for filtering relevant articles. As such, they may be effective for paper recommendations that are easy for researchers to quickly judge relevance of, but also bias them to snap judgment when the relevance is not easily established. 

Complementing such tailored strategies, modern day researchers also curate multiple channels for paper recommendations by selectively following relevant scholars on social networks such as Twitter and Academia.edu or by adopting RSS feeds and email alerts to receive personalized recommendations~\cite{van2014online,watkinson2016changes,tenopir2019changes}. However, the process of maintaining trusted sources of scholars are often deemed tedious, scattered, and relied upon chance discovery~\cite{breitinger2019too}. While tools that support these scholarly information behaviors have undergone drastic changes over time, the focus largely remained on advances in searching and indexing techniques, rather than providing sufficient explanations of relevance to researchers to help them engage with the recommendations. As Simon described, ``a wealth of information creates a poverty of attention,''~\cite{simon1996designing} and necessitates additional support situated in the current context of researchers' information behaviors to bridge the gap between retrieval of and engagement with paper recommendations.

% add something about current practices and how people heavily rely on heuristics such as venue, recency, citation counts, keyword match, guessing whether an article is a review or not by looking at how broad the keywords included in the title are, and opertaions to support those heuristics such as filter and sort....

% for relevant authors, also heuristics: authorship position

With this challenge in mind, we are motivated by the question: Can at-a-glance relevance information augmenting personalized paper recommendations enhance researcher engagement and sensemaking? This work takes a series of steps to uncover generalizable design implications for different types of at-a-glance relevance information, by focusing on the specific use context of paper recommendations received in user-subscribed email alerts. At a high level, there are contrasting notions of relevance in the literature on information need and perceived value of scholarly articles~\cite{case2016looking,belkin1985interaction} which we distinguish first. The logical notion of relevance, construed as aboutness or topicality (i.e. is the article on an appropriate topic as evidenced by containing specific terms?) differs from the user's holistic view of relevance which often emphasizes the notion of personalized usefulness. While the former focuses on content relatedness, the latter centers around users' subjective usefulness and broader information needs, which extend beyond the need for maximal content relatedness. For example, a researcher might find paper recommendations \textit{relevant} not because their content is directly related to a predefined research topic but because they are building off of the researcher's prior work, which she finds useful for understanding her work's impact in the field and ideating future research directions. Alternatively, she might find paper recommendations \textit{relevant} because of her social connection with one of the authors, as she is curious about what current and former colleagues are working on, and having a high-level understanding of their research trajectories gives her ideas for discussion, even if they are topically divergent. In yet another example, she might find paper recommendations useful because of the new authors she discovered from them, who she otherwise would not have encountered or paid enough attention to notice. As will be shown later, all of these examples involve usefulness outside the first notion of direct content relevance. In order to support such types of information needs, this work takes the broader, second perspective of relevance.\jb{This paragraph is much more helpful}

In this paper, we introduce three kinds of relevance information enabled by processing increasingly larger network structures of scholarly articles. The first kind (Citation-based relevance) presents relevance via citation using references included in new paper recommendations (e.g., This paper also cites 3 of your papers). Unlike older articles, these recommendations often lack incoming citations which constrains us to using references included in them. Citation relevance was also motivated by how researchers use bibliographic connections to search through the `back chains' of relevant prior work~\cite{barrett2005information,covi1999material,vakkari2006searching,westbrook2003information,bates2002speculations}.

Another kind (Direct author-based relevance) presents relevance via direct author-user relations (e.g., You cited the author 4 times), enabled by integrating author profiles into the citation network. This kind was motivated by how researchers typically follow work from a group of researchers known to them, for example on social media platforms such as Twitter or Academia.edu. The last kind (Indirect author-based relevance) presents relevance via indirect author-trusted scholar-user triplet relations (e.g., This author is often cited by a scholar you give credit to). To enable this, relations among the authors from the direct author relevance model are expanded to extract second-degree relations, mediated by the intermediate, trusted scholar. This was partly motivated by how researchers follow email discussion threads, use colleagues as information sources, or `cold email' high-profile experts in an outside field to receive highly valuable bibliography~\cite{vakkari2006searching,covi1999material,palmer2005scholarly,palmer2009scholarly}. It was also motivated by prior work in computational approaches for recommending content based on the social network of trusted sources~\cite{chen2010short,andersen2008trust}.\jb{The indirect author messages were motivated in large part by the success of author messages. Suggest reframing: we designed two graph-based explanations that explain connections to the user, which are useful in the alert setting where papers are ``fresh'' without incoming citations (also explain this setting earlier). Then, explain finding, which motivates the development of indirect messages} \jb{Thought: Are author messages a class of graph explanations where interaction is mediated by any node/relation - authors being one node, but could be venue, etc}

This paper begins with an iterative design process that involved several rounds of prototyping and informal evaluation with internal users and several relevant stakeholders. In total the process involved 7 users, a designer, a marketing person, and 3 researchers in AI and HCI. This iterative process resulted in the final message template designs for the first two types of relevance (citation- and direct author-based, Section~\ref{xx}). The message templates were filled in with personalized data and used to augment paper recommendations in new paper email alerts sent to users who subscribed to them. Given its use context, our message design's goals included brevity, visibility, and understandability. The final design (fig.~\ref{fig:xx}) adopted distinctive visual elements and colors, and was placed under each paper recommendation for easy access and low overhead for skimming.\jb{Too procedural for intro}

We then describe the procedure of a randomized online study which sought evidence for the feasibility of citation- and direct author-based relevance messages. While conducting design iterations and informal interviews provided initial qualitative insights into how relevance messages might support user engagement with new research article recommendations, without a large scale randomized experiment we were not able to quantify exactly how effective such methods were. In order to examine this, we ran a randomized online experiment with over seven thousand users on a popular scholarly search engine stretching over a two-month-period, by deploying personalized paper recommendations and relevance messages to alert email subscribers who were randomly assigned to each of the three conditions (Control vs. Citation-based vs. Direct author-based). Our result showed that both types of relevance messages significantly increased user engagement (24\% and 29\% increase over Control on the binary email click rates -- i.e. at least one click in the email -- using citation- and direct author-based messages, respectively. In addition, 145\% and 263\% increase over Control on the number of paper recommendations clicked per email that featured at least one relevance message, using citation- and direct author-based messages, respectively), but only author-based relevance messages resulted in a higher email open rate (13\% increase in email open rates over Control).

However, the effectiveness of relevance messages was hindered by their low frequency, and especially for author-based messages which on average resulted in less than 4\% of paper recommendations included in alert emails featuring relevance messages (in comparison, citation-based messages were significantly more common at around 9\%). Using logistic regression, we show that this limited frequency indeed seemed to have prevented broader engagement from users. Our third kind of relevance messages (Indirect author-based) was designed with the goal of increasing access to relevance messages in mind, and incorporated `endorsement' from a known intermediate author who the user may trust and would appreciate paper recommendations from. The choice of intermediate authors included those whose publications are highly relevant to those of the user, scholars who frequently co-authored with or were cited by the user as well as the authors of papers users frequently saved and liked in the past. The indirect author-based relevance messages then displayed the connection between the user and the intermediate author as well as the connection between the intermediate author and the author of the recommended paper. 

This work concludes with a controlled user study with fourteen researchers (Section~\ref{xx}). Researchers were observed as they reviewed four versions of paper recommendations -- the three kinds of relevance messages described above and Control. Researchers found different types of usefulness when interacting with paper recommendations augmented with relevance messages such as discovering new information about self and other authors to learn more, vetting potential usefulness of paper recommendations, mobilizing mental models of prior work and author expertise to better understand the recommendations, and as a general aid that increases user attention to others' work which was perceived useful for users' broader social context. We also uncover several design implications for future approaches including the tension between increased context and efficiency of skimming; adapting to users' evolving identities as researchers; and the challenges related to diffusion of relevance.

In summary, this work makes five contributions. First, we designed and implemented two types of relevance messages augmenting personalized paper recommendations, grounded in an iterative design process. Second, we present evidence from a large scale online deployment study that such an augmentation approach indeed increases user engagement. Third, we design and implement an additional kind of relevance messages that incorporates endorsement of paper recommendations through intermediate authors users likely know and give credit to. Fourth, we provide qualitative insights into how different types of relevance messages benefit users through a controlled lab study with fourteen researchers. Finally, we uncover design implications for future augmentation approaches that aim to incorporate relevance information.

\jb{Would be nice if we could explain how people who don't care about scholarly literature discovery can use our findings}

==> src4_study1_copy.tex <==
\subsection{Setting}
% Rafal: moved this to the beginning src3_message_design.tex

%We designed our online deployment study on a scholarly search engine. This engine provides users the ability to  search and curate interesting papers for personalized feeds. Users then can opt in to receive alert emails when new relevant papers are found for each feed on a regular basis, with a user selected frequency (e.g., daily or weekly). Typical alert emails start with a description of the feed the alert is generated for, and a list of papers (usually ranging from 1 to 50) found during the alert generation period, and other information and visual elements for saving the papers, managing the alert and so on (fig.~\ref{fig:email_alert} shows a simplified version). Some of the visual elements including paper titles are clickable and user engagement with them (e.g., clicking papers to check out the paper details page on the search engine website or opening emails) is recorded. This setting provides us an ideal ground for testing how users react different types of relevance messages, because users are given personalized paper recommendations that are predicted by the neural recommender as containing genuinely interesting and relevant content for curated feeds, thus providing us the ability to observe their authentic engagement patterns.

%\begin{wrapfigure}{R}{.45\textwidth}
%    \begin{center}
%    \includegraphics[width=.45\textwidth]{figures/email_alert_edit.png}
%    \caption{An abbreviated email alert is shown.}
%    \label{fig:email_alert}
%   \end{center}
%    % \vspace{-1em}
%\end{wrapfigure}



\subsection{Procedure} We randomly assigned about seven thousand users to one of the three conditions: Control/No message (status quo experience with the research feed and new paper alerts, without any relevance messages), Relevant-paper (citation-based relevance messages), and Relevant-author (author-based relevance messages) and sent out alert emails between April 7th, 2021 and June 13th, 2021. Table~\ref{table:email_stats} shows the number of users and emails sent in this period. Our main measure is click-through rates grouped at the email level (i.e. whether an email is opened and whether paper recommendations are clicked). 

\subsection{On reporting the results} We report the result of our studies below. To denote statistical significance we use the following notations: $^{*} (\alpha = 0.05)$, $^{**} (\alpha = 0.01)$, $^{***} (\alpha = 0.001)$, $^{****} (\alpha = 0.0001)$. Alpha levels are adjusted when appropriate in post-hoc analyses using Bonferroni correction.

\begin{wraptable}{R}{.7\textwidth}
    \centering
    \begin{tabular}{c c c c}
    \toprule
    \multirow{2}{*}{\textbf{Condition}} & \multirow{2}{*}{\textbf{\# of Users}} & \multirow{2}{*}{\textbf{\# of Emails}} & \textbf{\# of Emails with $\geq 1$} \\
    & & & \textbf{relevance message} (\% of total) \\
    \midrule
    Control & \fnum{2248} & \fnum{22548} & N/A\\
    Citation & \fnum{2474} & \fnum{23658} & \fnum{5984} (25\%) \\
    Direct Author & \fnum{2316} & \fnum{22657} & \fnum{3895} (16\%) \\
    \bottomrule
    \end{tabular}
    \caption{Descriptive statistics of the users and emails used for our analysis.}
    \label{table:email_stats}
\end{wraptable}

\subsection{Result}
\begin{figure}[t]
\begin{minipage}{.32\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/email_open_rates.png}
    \caption{The average email open rate was the highest in the Direct Author condition ($\mu=0.27$) followed by Citation ($\mu=0.24$) and Control ($\mu=0.24$). The differences between Relevant-author and two other conditions were significant at the $\alpha=0.05$ level after Bonferroni corrections for multiple tests.}
    \label{fig:open_rates}
\end{minipage}
\quad  
\begin{minipage}{.32\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/email_click_rates.png}
    \caption{The average email click rate was also the highest in the Direct Author condition ($\mu=0.058$) followed by Citation ($\mu=0.056$) and Control ($\mu=0.045$). The differences between Control and two other conditions were significant but not between the Relevant-paper and Relevant-author conditions.}
    \label{fig:click_rates}
\end{minipage}
\quad
\begin{minipage}{.24\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/email_click_rates_featured.png}
    \caption{However, when we account for different frequencies of relevance messages, Relevant-author messages ($\mu=0.16$) significantly outperformed Relevant-paper messages ($\mu=0.12$).}
    \label{fig:featured_click_rates}
\end{minipage}
\vspace{-1em}
\end{figure}

\subsubsection{Do relevance messages enhance user engagement with paper recommendation alert emails?} We found that both types of relevance messages significantly increased user engagement with emails. Comparing the overall email click rates between conditions, we found that Direct Author ($\mu=0.058, \bar{\sigma}=0.2330$, $t(44622.22)=6.20, p=5.6\times10^{-10}$) and Citation ($\mu=0.056, \bar{\sigma}=0.2292$, $t(46065.34)=5.36, p=8.3\times10^{-8}$) resulted in higher click-through rates than Control ($\mu=0.045, \bar{\sigma}=0.2068$) (Welch's two-tailed t-test with Bonferroni correction for multiple tests, fig.~\ref{fig:click_rates}), but the difference was not significant between the Citation and Direct Author conditions ($t(46149.07)=0.92, p=0.36$). However, only a fraction of the emails actually contained at least one paper recommendation with relevance message (25\% of the emails in the Citation condition and 16\% of the emails in the Direct Author condition, table~\ref{table:email_stats}) and because emails that did not feature any relevance message were virtually indistinguishable from emails in the Control condition, this was likely a lower bound estimate of messages' effectiveness. Therefore, we further estimated the engagement using a subset of emails that contained at least one relevance message. Using this subset of data, direct author-based messages led to a significantly higher average rate of click-through ($\mu=0.16, \bar{\sigma}=0.371$) than citation-based messages ($\mu=0.12, \bar{\sigma}=0.320$) (Welch's two-tailed t-test, $t(7445.46)=6.73, p=1.8\times10^{-11}$, fig.~\ref{fig:featured_click_rates}). These represent 268\% and 159\% increase over Control.

We further examined whether different message types resulted in differences in how often participants open the emails. If participants found the emails useful, they would open more of them in the future, resulting in a higher overall email open rates. In this sense, email open rates are indicative of future engagement. We found that the open rate was the highest in the Direct Author condition ($\mu=0.27, \bar{\sigma}=0.442$ vs. $\mu=0.24, \bar{\sigma}=0.428$ in Citation and $\mu=0.24, \bar{\sigma}=0.425$ in Control), and the difference was significant at the $\alpha=1.0\times 10^{-4}$ level. Citation and Control did not differ significantly. Because the titles, headers, or other metadata of emails did not differ between conditions, it is likely that the difference in open rates is attributed to the content of the emails and specifically the type of relevance messages featured in them.


\subsubsection{Post-hoc analyses on potential confounds of randomization}

\begin{wrapfigure}{R}{.6\textwidth}
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/mean_num_papers_per_email.png}
    \caption{The average length of emails were slightly shorter in Control ($\mu=12.1, \bar{\sigma}=20.30$) than the other two conditions ($\mu=12.9, \bar{\sigma}=21.74$ in Citation and $\mu=12.8, \bar{\sigma}=17.36$ in Direct Author), and the difference was less than one paper.}
    \label{fig:mean_email_length}
\end{minipage}
\quad  
\begin{minipage}{.25\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/mean_of_mean_ranks.png}
    \caption{The mean of mean position of relevance messages in emails was significantly higher in Direct Author than in Citation, suggesting an additional effort that direct author-based relevance message receivers had to exert to engage with them.}
    \label{fig:mean_of_mean_message_position}
\end{minipage}
\vspace{-1em}
\end{wrapfigure}

We further ran post-hoc analyses on two potential sources of confounds -- the average length of emails and the average position of relevance messages -- to ensure the validity of random assignment. Systemic differences in these confounds between conditions may significantly change user engagement, and have potential to invalidate the interpretation of the results on engagement. For example, longer emails may fatigue users and cause them to drop off more easily. At the same time, longer emails may also provide users more paper recommendations to look at, and as a result an increased click engagement. On the other hand, the average position of relevance messages would positively impact user discovery and attention, because messages placed higher (towards the top of the email) are more easily discovered. 

These potential sources of confounds seemed unlikely to have changed the directions of the observed effects on engagement. Though the length of emails \textit{did} significantly differ between conditions, and on average the emails in the Citation and Direct Author conditions were longer than in Control, this difference was less than a paper in both cases ($\Delta_{\text{Citation} - \text{Control}}=0.78$ and $\Delta_{\text{Direct Author} - \text{Control}}=0.69$). The average number of paper recommendations clicked per email was $\mu=0.10, \bar{\sigma}=0.680$, the expected number of clicked emails from the difference is then $0.78\times0.10=0.078$ for the Citation condition and $0.69\times0.10=0.069$ for the Direct Author condition. However, the average number of clicked emails in both treatment conditions were still higher after accounting for the expected surpluses of clicked papers, $\mu=0.24, \bar{\sigma}=0.936$ (Citation) and $\mu=0.36, \bar{\sigma}=1.262$ (Direct Author). Between the Citation and Direct Author conditions, the average position of relevance messages indexed from the top of the email was lower (i.e. closer to the top of the email) in the Citation condition ($\mu=10.1, \bar{\sigma}=20.55$) than in the Direct Author condition ($\mu=12.0, \bar{\sigma}=17.72$). This suggests that if the discoverability of relevance messages were controlled for, Direct Author messages may lead to an even higher level of increase on user engagement.

\subsubsection{How did featuring relevance messages change whose paper recommendations get clicked?} \label{section:h-index-analysis} Though effective, featuring paper recommendations with relevance messages might also produce unanticipated negative externalities such as boosting the visibility of papers by authors who are already commonly featured in the recommender system. The phenomenon of ``rich-get-richer'' has been widely studied in scholarly domains~\cite{cole1968visibility,bol2018matthew,merton1968matthew,price1976general,crane1965scientists,judge2007causes,lariviere2010impact,medoff2006evidence,diprete2006cumulative,van2014field,wang2014unpacking}, but how scientific recommender systems may influence the visibility of certain work and authors has not been systematically studied thus far.

\begin{figure}[t]
\begin{minipage}{.20\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/all_max_h.png}
    \caption{The `background' distribution of max author h-index from each paper recommendation sent out in all alert emails in all conditions. $\mu=18.0, \bar{\sigma}=23.29$ (median=$9.0$).}
    \label{fig:all_normalized_h}
\end{minipage}
\qquad  
\begin{minipage}{.63\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/treatment_max_h.png}
    \caption{The distribution of max author h-indices of clicked papers in each condition. The average increased to $\mu=27.0, \bar{\sigma}=29.33$ (Control, median=$17.0$); $\mu=23.1, \bar{\sigma}=24.24$ (Citation, median=$16.0$); and $\mu=26.4, \bar{\sigma}=26.67$ (Direct Author, median=$18.0$). The significant increases of h-indices of authors of clicked papers suggest that users (at least partially) considered high h-index authors as a signal for deciding to click on a paper. Both Citation and Direct Author conditions shifted the h-index distribution less or to a similar extent relative to Control.}
    \label{fig:clicked_normalized_h}
\end{minipage}
\vspace{-1em}
\end{figure}

One way to examine relevance messages' effect on visibility is to take an outcome oriented approach, by measuring changes on the paper links users clicked before and after augmenting the recommendations with messages. When a user clicks on a paper link, it brings her to a webpage dedicated to the paper which includes additional information about the paper such as its full abstract, the link to a full-text file, any figures, and the author information among others. Users may choose to further interact with any visual elements on the page. Therefore the click serves as a strong indicator of user's exposure to the paper's content. We then operationalize the visibility for each paper as a binary measure of whether it is clicked; when a paper is clicked for the first time, it is made visible to the user. Using this measure of visibility, we are interested in investigating whether its distribution among the authors with varying academic status systematically changes after the introduction of relevance messages. 

We operationalized the academic status of each author using the h-index measure. The index, since its introduction by Hirsch in 2005~\cite{hirsch2005index}, has been popularized as a metric of academic success. Though limitations of the index exist~\cite{panaretos2009assessing,sinatra2016quantifying}, it is seen as a robust measure~\cite{hirsch2007does,radicchi2008universality,henzinger2010stability,acuna2012predicting}, and informs high stakes decisions such as hiring, promotion, and funding~\cite{mcnutt2014measure,hicks2015bibliometrics,abbott2010metrics}. It is also widely featured in many scholarly search engines and citation databases.

To examine whether relevance messages led to users clicking papers featuring high status authors more often, we first assigned an h-index to each paper recommendation by taking the max h-index of authors, and aggregated it over all recommendations sent out in alert emails. This produced our baseline h-index distribution of authors (fig.~\ref{fig:all_normalized_h}). Next, we similarly computed the h-index of each recommendation but using only the clicked paper recommendations from each condition (fig.~\ref{fig:clicked_normalized_h}). Finally, we tested whether the average h-index of clicked papers significantly differed from that of the baseline. The result showed that the distribution indeed significantly shifted to the right for clicked papers with or without relevance messages, suggesting that users incorporate author names (and subsequently their h-indices) when deciding whether to click on a paper recommendation. However, the shift was the largest in Control, suggesting the signal from author names is weighted higher in the absence of relevance messages ($\mu=8.3 \rightarrow \mu=12.5$, $t(2254.88)=13.69, p=0$, Welch's two-tailed t-test). Citation showed a significantly lower increase than Control ($t(4187.11)=4.66, p=3.26\times10^{-6}$). The increase in Direct Author did not statistically significantly differ from Control ($t(4401.29)=0.87, p=0.38$). Furthermore, one may also hypothesize that users incorporate signals from multiple author names by averaging them when making a decision to click on a paper recommendation. To evaluate this hypothesis, we also tested whether assigning each paper an average h-index from its authors changed the patterns of distributional shifts. Our results showed that the patterns remained the same (see Appendix). Taken together, we conclude that augmenting paper recommendations did not exacerbate the issue of the fairness of visibility, and may have helped when citation-based relevance messages are used.

\subsubsection{How did the frequency of relevance messages differ between conditions?} \label{subsubsection:study1-frequency}

\begin{figure}[t]
\begin{minipage}{.20\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/avg_featured_papers.png}
    \caption{The number of papers featured with relevance messages was significantly higher in Citation ($\mu=1.3$) than in Direct Author ($\mu=0.5$).}
    % The number of papers featured with relevance messages was significantly higher in Citation ($\mu=1.3, \bar{\sigma}=7.37$) than in Direct Author ($\mu=0.5, \bar{\sigma}=1.85$) ($t(26739.0)=16.6, p=0$, Welch's two-tailed t-test).
    \label{fig:avg_num_featured_papers}
\end{minipage}
\quad
\begin{minipage}{.20\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/avg_featured_papers_normalized.png}
    \caption{The \% of papers featured with relevance messages was similarly higher in Citation ($\mu=0.09$) than in Direct Author ($\mu=0.04$).}
    % When normalized by the length of emails, the fraction of papers featured with relevance messages was similarly higher in Citation ($\mu=0.09, \bar{\sigma}=0.212$) than in Direct Author ($\mu=0.04, \bar{\sigma}=0.119$) ($t(37428.4)=31.9, p=0$, Welch's two-tailed t-test).
    \label{fig:avg_frac_featured_papers}
\end{minipage}
\quad
\begin{minipage}{.5\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/avg_fraction_featured_h_group.png}
    \caption{Recipients in the low h-index group received emails with less Direct Author relevance messages ($\mu=0.09$) than the high index group ($\mu=0.18$). The frequency of citation-based relevance messages did not differ significantly between Low and High index groups, suggesting a relative abundance of citation relations compared to author-focused relations.}
    % Dividing email recipients into three groups of h-index (Low, High, and Unknown) using the median of known indices, the low index group received emails with less Direct Author relevance messages ($\mu=0.09$) than the high index group ($\mu=0.18$, $p=1.3\times10^{-18}$), but more than the index unknown group ($\mu=0.03$, $p=3.7\times10^{-20}$). Because h-index is computed for users with claimed profiles on the search engine, this set of users are expected to be more engaged with the engine and hence richer in data. Therefore, low frequencies of relevance messages are expected. Surprisingly, the frequency of citation-based relevance messages did not significantly differ between Low and High index groups, suggesting a relative abundance of citation relations compared to author-focused relations.
    \label{fig:avg_frac_featured_papers_h_group}
\end{minipage}
\vspace{-1em}
\end{figure}

Despite the higher effectiveness of author-based relevance messages, they were rarer ($\mu=0.5, \bar{\sigma}=1.85$) than citation-based messages ($\mu=1.3, \bar{\sigma}=7.37$, $t(26739.0)=-16.6, p=0$, Welch's two-tailed t-test) (fig.~\ref{fig:avg_num_featured_papers}). The pattern remained similar when normalized by the length of emails  ($\mu=0.09, \bar{\sigma}=0.212$ in Citation vs. $\mu=0.04, \bar{\sigma}=0.119$ in Direct Author, $t(37428.4)=31.9, p=0$). Further dividing email recipients into three groups of h-index (Low, High, and Unknown) using the median (3) of h-indices from a small number of authors whose h-indices were available (h-index was known for 115 out of \fnum{2474} users in the Citation condition and 107 out of \fnum{2316} users in the Direct Author condition), the low index group received emails featuring less Direct Author relevance messages ($\mu=0.09, \bar{\sigma}=0.183$) than the high index group ($\mu=0.18, \bar{\sigma}=0.228, p=1.3\times10^{-18}$). However, compared to the index unknown group, the low index group still received emails featuring more Direct Author relevance messages than ($\mu=0.09 > \mu=0.03, \bar{\sigma}=0.104, p=3.7\times10^{-20}$) (fig.~\ref{fig:avg_frac_featured_papers_h_group}). This is not surprising given that the h-index is computed only for users with claimed profiles on the search engine, and because this set of users is expected to be overall more highly engaged with the system and have richer interaction data available for the recommender system to generate relevance messages from.

As shown in fig.~\ref{fig:avg_frac_featured_papers_h_group}, only the high h-index group of users received a similar fraction of relevance messages for both types of relevance (Welch's two-tailed t-test was not significant at the $\alpha=0.05/6$ level after correcting for multiple tests $t(1522.6)=-2.45, p=0.014$). For the rest of the users, author-based relevance messages was a rare occurrence. Furthermore, the frequency of citation-based relevance messages did not significantly differ between Low and High index groups, suggesting a relative abundance of citation-based relations for users with less publications, but not author-based relations. Taken together with the earlier results on the effectiveness of author-based relevance messages, these results suggest increasing their frequency may further encourage users to engage with paper recommendations. However it is unclear how many more relevance messages would produce positive effects on user engagement before losing value as a signal or overwhelming the user.

\subsubsection{How does the \% of papers featured with author-based relevance messages effect changes on user engagement?}

\dd{These first two paragraphs are my attempt at a shortened version of this section.  I'm realizing this may be too drastic of a change so I am going to leave everything else in place, but I think we could get away with this change.}

We now show evidence that even after controlling for multiple confounds, engagement increases with the number of papers featured in the mail.
First, as shown in Figure \ref{fig:clicked_by_fraction_featured}, empirically we find that emails with a greater fraction of treated papers result in dramatically more engagement (in terms of clicked emails), up to a point (between 25-50\% treated) above which engagement falls off.  However, the amount of engagement also varies significantly with other potentially confounding factors that also correlate with the fraction of featured papers.  For example, users with a higher h-index and a claimed profile have more user data in the system that can be used to feature a larger fraction of papers---and these users also tend to show higher engagement (see Figures \ref{fig:clicked_by_h} and \ref{fig:clicked_by_claimed_profile}).  

We investigated these confounds in the form of a mixed effects model (details in Table \ref{table:dataset}).  The results, shown in Table \ref{table:glmm2}, show that a significant negative quadratic dependence of engagement on the percentage of featured papers, even in the presence of other potential predictors like whether the profile is claimed, and the receiver's h-index.  The estimated effects, according to this model, of different fractions of treated mails in different conditions (including as another variable, the number of papers per email, varies) are shown in Figure \ref{fig:estimated_overall}.
This analysis suggests that for users with less interaction history and fewer featured papers, strategies to increase their fractions of featured papers to the 25-50\% range are a promising method for increasing engagement.  We turn to these strategies in the next section.

\dd{end Doug edits, original text follows}

Since the fraction of papers that can be treated using the techniques described in previous sections is limited by the amount of user activity, this spurred us to 

\xhdr{Dataset Structure} In order to home in on the effect of the \% of papers featured with author-based relevance messages on email-level user engagement, we prepared the data from the Direct Author condition in the deployment study (\fnum{22657} emails from \fnum{2316} users over a two-month-long period) for regression analysis as follows (table~\ref{table:dataset}).

\begin{table}[t]
    \centering
    \begin{tabular}{@{\extracolsep{4pt}}c c c c c c c}
    \toprule
    \multirow{3}{*}{Receiver ID} & \multirow{3}{*}{Mail ID} & Dep. Variable & \multicolumn{4}{c}{Predictive Variables} \\
    \cline{3-3}\cline{4-7}
     &  & \multirow{2}{*}{Email Clicked} & Claimed & \multirow{2}{*}{Receiver h-index} & \multirow{2}{*}{\% Featured} & \# of Total\\
     &  &  & Profile &        &    & Papers\\
    \midrule
    1 & 100 & 1 & 1 & 3 & 0.38 & 14 \\
    2 & 101 & 1 & 0 & 11 & 0.60 & 20 \\
    1 & 102 & 0 & 1 & 3 & 0.30 & 10 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Sample format of the data collected from the online deployment study.} Each row represents a unique user - alert email combination. \textit{Email Clicked} is the binary dependent variable representing the email-level user engagement outcome. \textit{Claimed Profile} shows whether the user has a claimed profile on the search engine, an indication of a generally high-level engagement. \textit{Receiver h-index} shows the h-index of the receiver and was normalized before the analysis. \textit{\% Featured} shows the \% of paper recommendations in the email augmented with author-based relevance messages. \textit{\# of Total Papers} shows the total number of papers included in the email and was normalized before the analysis.}
    \label{table:dataset}
\end{table}

%\xhdr{Analytic Framework}

\begin{wrapfigure}{R}{.3\textwidth}
    \begin{center}
    \includegraphics[width=.3\textwidth]{figures/email_clicked_fraction_featured.png}
    \caption{Empirical data on the change of the rate of clicked emails from \% featured suggests an inverted U-shaped curve relation.}
    \label{fig:clicked_by_fraction_featured}
    \end{center}
    % \vspace{-1em}
\end{wrapfigure}

We analyzed our dataset using generalized linear mixed-effects (GLMM) models with the \textsc{lme4} package in R~\cite{bates2014fitting}. The dependent variable (\textit{Email Clicked}) is binary (0: email with zero click on paper recommendations, 1: email with at least one click on paper recommendations), and fixed effects as a function of \textit{Claimed Profile}, \textit{Receiver h-index}, \textit{\% Featured}, and \textit{\# of Total Papers} (normalized)\footnote{We also considered Generalized Estimating Equations (GEE)~\cite{liang1986longitudinal} as an alternative analytical framework to GLMM. GEE is used in various application domains involving longitudinal data~\cite{hubbard2010gee,odueyungbo2008comparison,ballinger2004using,ma2012beyond,hu1998comparison}, and may be useful in our case for accounting for correlation within groupings of similar individuals beyond just correlation across multiple observations from a single individual. However, grouping structures of similar individuals in our dataset is beyond the scope of this work}. 
We also introduced a random effect with \textit{Receiver ID} to capture correlation across each individual's engagement responses across multiple emails (see Appendix~\ref{appendix:GLMM} for more details about the how we decided to include these factors into modeling).

\xhdr{The curvilinear relation between the \% of papers featured with author-based relevance messages and user engagement}

We hypothesized that an optimal \% of papers within an email featured with author-based relevance messages is neither too few -- which may lead to under-utilization, nor too many -- which may lead to overwhelming the users. Investing this curvilinear relation requires inclusion of a quadratic variable in the model. The descriptive pattern from the data also suggested this hypothesis (fig.~\ref{fig:clicked_by_fraction_featured}). Using locally weighted scatterplot smoothing (\textsc{LOWESS}), we see that the peak engagement happened somewhere between 25\% and 50\% of the papers featured with author-based relevance messages, and quickly decreases outside this range. In addition to the descriptive pattern from the data,  we also first performed a pairwise Likelihood Ratio Test (LRT) on two models (see Appendix~\ref{appendix:GLMM} for more details on model configuration), one with a linear \% Featured term but no quadratic term, and the other with a quadratic $\left(\text{(\% Featured)}\right)^2$ term but no linear term, in order to further test the soundness of introducing the quadratic term. The result showed that the reduction of deviance from introducing the quadratic term is more than what we would have expected to see if the beta coefficients for them were 0 ($\chi^2(1)=19.9, p=8.1\times10^{-6}$), thus we proceeded with introducing the quadratic term and building Model 1\footnote{We did not perform an additional check on the VIF when including the quadratic term, despite its potentially significant collinearity with the linear term. See~\cite{o2017dropping} for more discussion on the relevant topic.}.

\begin{wraptable}{R}{.4\textwidth}
    \centering
    \begin{tabular}{@{\extracolsep{4pt}}c c c c}
    \toprule
     & Coef. & SE & $p$ \\
    \midrule
    (Intercept) & -8.2016 & 0.2777 & *** \\
    $\text{\% Featured}$ & 3.1686 & 0.5977 & *** \\
    $\left(\text{\% Featured}\right)^2$ & -2.9980 & 0.6798 & *** \\
    \# of Total Papers & 0.0092 & 0.0381 & 0.81 \\
    \bottomrule
    \end{tabular}
    \caption{Regression analysis using Model 1 predicts change in user engagement given a quadratic function of the \% of papers featured with author-based relevance messages, and the total number of paper recommendations included in the email. *** indicates significance at $p<0.001$.}
    \label{table:glmm1}
    \vspace{-1em}
\end{wraptable}

The result of Model 1 regression analysis is shown in Table~\ref{table:glmm1}. This regression tells us whether the probability of user engagement changes significantly if we increased the \% of papers featured with author-based relevance messages, or changed the number of paper recommendations included in each email. Consistent with our hypothesis, we found a significant curvilinear relationship between the \% of papers featured in the email and the user engagement. The coefficients of both the linear \% Featured and its quadratic terms were significant ($p<0.001$), and the signs were in the opposite direction, with a negative beta coefficient for the quadratic term. This indicates an inverted U-shaped curve relation on user engagement from the fraction of papers featured in the email. We also found that the normalized length of email was not a significant predictor of user engagement. This may due to the conflicting effects of longer emails: overwhelming users (negative) vs. providing more paper links to click (positive). 

\xhdr{Factors related to adaptive strategies}

\hyeonsu{Move these two plots to Appendix}

\begin{figure}[t]
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{figures/email_clicked_normalized_h_index.png}
    \caption{Empirical data on the change of the rate of clicked emails from normalized receiver h-index. The receiver h-index is significantly positively associated with email click engagement.}
    \label{fig:clicked_by_h}
\end{minipage}
\quad  
\begin{minipage}{.6\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/email_clicked_claimed_profile_facet.png}
    \caption{Empirical data on the change of the rate of clicked emails from \% featured, faceted by whether the user claimed a profile or not. Users with claimed profiles show higher levels of engagement as the \% featured increases, suggesting a potential }
    \label{fig:clicked_by_claimed_profile}
\end{minipage}
\vspace{-1em}
\end{figure}

In the previous section we showed that increasing the \% of papers featured with author-based relevance messages positively influences user engagement, but only up to a certain extent. This curvilinear relation might be further influenced by contextual factors related to user-specific information, such as the academic status or the general level of engagement with the system, or the length of the email. Estimating from such factors can inform us future strategies for fine-tuning how often paper recommendations are featured with relevance information, based on the user- and email-specific information and preferences.

\begin{wraptable}{R}{.6\textwidth}
    \centering
    \begin{tabular}{@{\extracolsep{4pt}}c c c c}
    \toprule
     & Coef. & SE & $p$ \\
    \midrule
    (Intercept) & -7.76786 & 0.28246 & *** \\
    $\text{\% Featured}$ & 4.56360 & 0.82277 & *** \\
    $\left(\text{\% Featured}\right)^2$ & -4.95201 & 1.06339 & *** \\
    \# of Total Papers & 0.01591 & 0.03764 & 0.67248 \\
    Claimed Profile & 2.26396 & 0.34874 & *** \\
    Receiver h-index & 9.53340 & 3.47593 & ** \\
    $\text{\% Featured}$ $\times$ Claimed Profile & -3.41986 & 1.28354 & ** \\
    $\left(\text{\% Featured}\right)^2$ $\times$ Claimed Profile & 4.29778 & 1.49945 & ** \\ 
    $\text{\% Featured}$ $\times$ Receiver h-index & -2.25113 & 5.55917 & 0.68552 \\
    $\left(\text{\% Featured}\right)^2$ $\times$ Receiver h-index & 2.00482 & 7.82939 & 0.79790 \\
    \bottomrule
    \end{tabular}
    \caption{Regression analysis with Model 2 predicts change in user engagement given the predictive variables in Table~\ref{table:glmm1} as well as additional factors of user ownership of a profile, her h-index, and the two-way interactions with $\text{\% Featured}$ and $\left(\text{\% Featured}\right)^2$. ***: $p<0.001$, **: $p<0.01$, *: $p<0.05$.}
    \label{table:glmm2}
    \vspace{-1.5em}
\end{wraptable}

We first examined how the rate of clicked emails changes based on user-specific information in our data. Fig.~\ref{fig:clicked_normalized_h} shows that the normalized receiver h-index is positively correlated with the click-through rates. Note that individuals with higher h-index are also correlated with the higher amount of available data in the system, as we saw previously in fig.~\ref{fig:avg_frac_featured_papers_h_group}. In addition, whether the user claimed a profile was also associated with the relation between the rate of clicked emails and the \% of papers featured. Specifically, for a user with claimed profile (fig.~\ref{fig:clicked_by_claimed_profile}, right), the level of engagement remained high as the \% featured increased beyond 50\% relative to a user without a claimed profile. This suggests an effect from the interaction between Claimed Profile and \% Featured.

Based on these observations, we introduced the following factors into Model 1 to build an expanded Model 2: a binary variable indicating whether the user has a profile on the search engine; the h-index of the receiver; and these two factors' interaction with \% Featured as well as its quadratic term. The result of regression analysis is shown in Table~\ref{table:glmm2}. With the new variables and interaction terms added, the estimated beta coefficients of the overlapping factors with Model 1 changed but not their signs nor levels of significance, consistent with the results from Model 1. We found that the Claimed Profile variable is significantly positively associated with user engagement (beta=2.26, Z=6.492, $8.5\times10^{-11}$), showing that users with claimed profiles indeed showed an overall higher level of engagement than those without profiles. We also found a significant positive interaction effect from $\text{\% Featured}\times$Claimed Profile (beta=-3.42, Z=-2.664, $p=0.008$) and $\left(\text{\% Featured}\right)^2\times$Claimed Profile (beta=4.30, Z=2.866, $p=0.004$). This indicates a diminishing return from the combination beyond the optimal \% featured, while also an increasing return below the optimal \% featured. Finally, the normalized receiver h-index was also significantly positively associated with Clicked Email (beta=9.53, Z=2.743, $p=0.006$). However, unlike Claimed Profile the factor did not indicate any interaction effect with the \% featured. 

\begin{figure}[t]
\begin{minipage}{\textwidth}
    \includegraphics[width=.22\textwidth]{figures/estimated_likelihood_overall.png}
    \includegraphics[width=.22\textwidth]{figures/estimated_likelihood_n=10.png}
    \includegraphics[width=.22\textwidth]{figures/estimated_likelihood_n=20.png}
    \includegraphics[width=.28\textwidth]{figures/estimated_likelihood_n=30.png}
    \caption{\textbf{Estimated changes on the marginal likelihood of clicked emails.} The overall estimated marginal click likelihood by \% of featured papers (1st figure); The estimated click likelihood by \% of featured papers in an average email of length 10 (2nd figure); 20 (3rd figure); and 30 (4th figure).}
    \label{fig:estimated_overall}
\end{minipage}
\vspace{-1em}
\end{figure}

In addition to the user-specific information, other contextual factors such as the overall length of emails might influence the effectiveness of relevance messages. We first estimated the optimal \% featured for author-based relevance messages for the overall data (fig.~\ref{fig:estimated_overall}) with the population average. The peak likelihood of email clicks formed around 50\%. Next, similar analyses on the data subset by the length of the emails ($N=10, 20, 30$) revealed a pattern that shows how the total length of emails might interact with \% featured. For example as the length of emails increased, the distribution shifted to the left, suggesting that the optimal \% featured within an email before diminishing returns depends on this contextual factors.


% \xhdr{What is the estimated optimal \% of papers featured with author-based relevance messages?}

% We built a series of logistic regression models involving an increasing number of factors to answer our research question. At each step of introducing additional factors in the model we recorded if the predicted signs or levels of significance on factors from earlier models changed significantly. A detailed description of the process can be found in Appendix~\ref{appendix:logit}. We also included quadratic terms of certain independent variables in the regression model when necessary. Following~\cite{o2017dropping}, we do not include such power terms in the VIF

==> zz_sleepingkittens.tex <==
% \begin{figure}[t]
%     \includegraphics[height=0.21\textheight]{figures/avg_featured_papers.png}
%     \caption{}
%     \label{fig:click_rates}}
% \vspace{-1em}
% \end{figure}

% \begin{figure}[t]
% \subfloat[]{%
%     \includegraphics[height=0.21\textheight]{figures/avg_featured_papers.png}
%     \label{fig:click_rates}}
% \quad
% \subfloat[]{%
%     \includegraphics[height=0.21\textheight]{figures/avg_featured_papers_normalized.png}
%     \label{fig:open_rates}}
% \vspace{-1em}
% \caption{}
% \end{figure}


% \begin{figure}[t]
% \subfloat[]{%
%     \includegraphics[height=0.21\textheight]{figures/avg_featured_papers.png}
%     \label{fig:click_rates}}
% \quad
% \subfloat[]{%
%     \includegraphics[height=0.21\textheight]{figures/avg_featured_papers.png}
%     \label{fig:click_rates}}
% \quad
% \subfloat[]{%
%     \includegraphics[height=0.21\textheight]{figures/avg_featured_papers_normalized.png}
%     \label{fig:open_rates}}
% \vspace{-1em}
% \caption{}
% \end{figure}


% \begin{minipage}{\linewidth}
%     \centering
%     \begin{minipage}{0.45\linewidth}
    
%     \end{minipage}
%     \begin{minipage}{0.45\linewidth}
    
%     \end{minipage}
% \end{minipage}
